Towards Understanding and Quantifying Uncertainty for Text-to-Image Generation

Uncertainty quantification in text-to-image (T2I) generative models is crucial for understanding model behavior and improving output reliability. In this paper, we are the first to quantify and evaluate the uncertainty of T2I models with respect to the prompt. Alongside adapting existing approaches designed to measure uncertainty in the image space, we also introduce Prompt-based UNCertainty Estimation for T2I models (PUNC), a novel method leveraging Large Vision-Language Models (LVLMs) to better address uncertainties arising from the semantics of the prompt and generated images. PUNC utilizes a LVLM to caption a generated image, and then compares the caption with the original prompt in the more semantically meaningful text space. PUNC also enables the disentanglement of both aleatoric and epistemic uncertainties via precision and recall, which image-space approaches are unable to do. Extensive experiments demonstrate that PUNC outperforms state-of-the-art uncertainty estimation techniques across various settings. Uncertainty quantification in text-to-image generation models can be used on various applications including bias detection, copyright protection, and OOD detection. We also introduce a comprehensive dataset of text prompts and generation pairs to foster further research in uncertainty quantification for generative models. Our findings illustrate that PUNC not only achieves competitive performance but also enables novel applications in evaluating and improving the trustworthiness of text-to-image models.

==> sec/figuretikz.tex <==
\begin{tikzpicture}[
  box/.style={
    draw=gray, thick, line width=1mm, rounded corners,
    text width=4.5cm, align=center, minimum height=4.5cm, font=\sffamily\Large
  },
  thinbox/.style={
    draw=gray, thick, line width=1mm, rounded corners,
    text width=3.5cm, align=center, minimum height=2cm, font=\sffamily\Large
  },
  arrow/.style={-{Latex}, thick, line width=1mm, draw=gray},
  dashedline/.style={dashed, draw=gray, line width=1mm},
  tallbox/.style={
    draw=gray, thick, line width=1mm, rounded corners,
    text width=10cm, align=center, minimum height=3cm, font=\sffamily\Large
  }
]

% Top section with model flow
\node[box, fill=blue!10] (prompt) {Concepts in prompt: \texttt{Japanese man, Kishida Fumio, holding, fish, white shirt}};
\node[thinbox, right=1cm of prompt, fill=blue!35] (model) {Text-to-image model};
\node[thinbox, right=1cm of model, fill=green!35] (image) {Image};
\node[box, right=1cm of image, fill=green!10] (concepts) {Concepts in generation: \texttt{Japanese man, holding, fish, white shirt, carp, smiling}};

\draw[arrow] (prompt) -- (model);
\draw[arrow] (model) -- (image);
\draw[arrow] (image) -- (concepts);

% Dashed dividing line
\draw[dashedline] ($(model.south west) + (-5.5,-2)$) -- ($(image.south east) + (5.5,-2)$);

% Bottom section with equations
% \node[tallbox, below=5cm of $(model.west) + (-0.5,0)$, fill=gray!30] (recall) {\textcolor{red!50!white}{\textit{Epistemic}}\\Recall-based Uncertainty\\~\\\huge{$\frac{\text{\#concepts from prompt in generation}}{\text{\#concepts in prompt}} = \frac{3}{4}$}};
\node[tallbox, below=4.5cm of prompt.east, fill=gray!30] (recall) {\textcolor{red!50!white}{\textit{Epistemic}}\\ \underline{Recall}-based Uncertainty\\~\\\huge{$\frac{\text{\#concepts in \textcolor{green!70!black}{generation} from \textcolor{blue!70}{prompt} }}{\text{\#concepts in \textcolor{blue!70}{prompt}}} = \frac{4}{5}$}};
\node[tallbox, right=0.5cm of recall, fill=gray!10] (precision) {\textcolor{red!50!white}{\textit{Aleatoric}}\\ \underline{Precision}-based Uncertainty\\~\\\huge{$\frac{\text{\#concepts in \textcolor{green!70!black}{generation} from \textcolor{blue!70}{prompt} }}{\text{\#concepts in \textcolor{green!70!black}{generation}}} = \frac{4}{6}$}};

% Centering section labels
\node[above=1.5cm of $(prompt)!0.5!(concepts)$, font=\bfseries\Large\sffamily] (label_top) {Image Generation Model Flow};
\node[below=3.5cm of $(prompt)!0.5!(concepts)$, font=\bfseries\Large\sffamily] (label_bottom) {Semantic Concept Uncertainty Quantification};

\end{tikzpicture}
